A deep survey of short GRB host galaxies over $z\sim0-2$: implications for offsets, redshifts, and environments

A significant fraction (30\%) of well-localized short gamma-ray bursts (sGRBs) lack a coincident host galaxy. This leads to two main scenarios: \textit{i}) that the progenitor system merged outside of the visible light of its host, or \textit{ii}) that the sGRB resided within a faint and distant galaxy that was not detected by follow-up observations. Discriminating between these scenarios has important implications for constraining the formation channels of neutron star mergers, the rate and environments of gravitational wave sources, and the production of heavy elements in the Universe. In this work, we present the results of our observing campaign targeted at 31 sGRBs that lack a putative host galaxy. Our study effectively doubles the sample of well-studied sGRB host galaxies, now totaling 72 events of which $28\%$ lack a coincident host to deep limits ($r$\,$\gtrsim$\,$26$ or $F110W$\,$\gtrsim$\,$27$ AB mag), and represents the largest homogeneously selected catalog of sGRB offsets to date. We find that 70\% of sub-arcsecond localized sGRBs occur within 10 kpc of their host's nucleus, with a median projected physical offset of $5.6$ kpc. Using this larger population, we discover an apparent redshift evolution in their locations: bursts at low-$z$ occur at $2\times$ larger offsets compared to those at $z$\,$>$\,$0.5$. This evolution could be due to a physical evolution of the host galaxies themselves or a bias against faint high-$z$ galaxies. Furthermore, we discover a sample of hostless sGRBs at $z$\,$\gtrsim$\,$1$ that are indicative of a larger high-$z$ population, constraining the redshift distribution and disfavoring log-normal delay time models.

==> O'Connor et al. Host Galaxies Paper/new_disc_tes.tex <==
\nora{
2) There is a lingering ambiguity in the origin of hostless events. For instance, 
the sample of Berger lies close to nearby galaxies and could be either highly offset or high redshift. This works finds a large fraction of hostless events NOT associated to any nearby galaxy, but either faint or undetected hosts. 
Therefore we can say that XX per cent of hostless are likely high-z events.
3) We also examine the sample of hostless events that do lie close to a nearby galaxy, and in particular use their high-energy properties to probe their environment.  We do find a trend correlating the brightness of the X-ray afterglow with the GRB location, being large offset events also X-ray faint. 
We note that X-ray constraints of hostless events are either too shallow or not consistent with the observed trend.  Although this does not conclusively rule out that these hostless GRBs could be mergers kicked out in the IGM, it does not offer observational support and leave their nature undetermined. 
The most critical observational tests would be: 1) rapid afterglow spectroscopy (16410A), to
determine the distance scale directly from the afterglow. 2) rapid and deep X-ray observations, capable of probing X-ray fluxes of 1e-16 within 12 hrs since the GRB. 
This is ATHENA but it is not expected to fly for the next 12 years! 3) detect a kilonova which would provide an indirect evidence of a low-z due to their maximum peak luminosity (Chase et al...)
}


We emphasize that there is a lingering ambiguity as to the origin of hostless short GRBs. For instance, the hostless sGRBs presented by \citet{Berger2010a} are located at a significant offset ($30$\,$-$\,$75$ kpc) from bright low-$z$ ($z<0.5$) galaxies. However, despite their brightness, the probability of chance coincidence is $\gtrsim 10\%$. Therefore, it is not clear whether these sGRBs are truly associated to these low-$z$ galaxies, or whether they reside in faint, undetected host galaxies. 

In this work, we have tripled the number of observationally hostless sGRBs (from 7 to 20 events). We instead uncovered a population of 9 observationally hostless sGRBs (see \S \ref{sec: hostlum}) without any nearby (low-$z$) candidate host galaxy. As such, these events are more likely to have exploded in faint $r\gtrsim 24.5$ mag galaxies, which are consistent with $0.1-1.0L^*$ galaxies at $z>1$. Therefore, we set a lower limit of $>45\%$ to the fraction of hostless sGRBs at high-$z$.

A larger population of sGRBs at $z$\,$>$\,$1$ implies a steep DTD with an increased fraction of events with short delay times, as deduced based on Galactic BNS systems \citep[][]{BeniaminiPiran2019}. We note, however, that an alternative explanation is that these are due to a population of low luminosity ($<$\,$0.1 L^*$) galaxies hosting sGRBs at $z$\,$<$\,$1$, although this at tension with the population of well-determined sGRB hosts ($0.1$\,$-$\,$1 L^*$; \citealt{Berger2010a}) and with predictions from population synthesis modeling, which find that BNS systems preferentially form in the most massive (brightest) galaxies \citep{Behroozi2014,Mapelli2018,Artale2019,Artale2020,Adhikari2020,Mandhai2021,Chu2022}. 

We further explored the sample of observationally hostless events that lie close to low-$z$ galaxies. We exploited their high-energy properties to probe their environments (\S \ref{sec: environment}). Figure \ref{fig: fluxfluence_vs_offset} shows a weak correlation between the brightness of the X-ray afterglow with the sGRB location, such that a larger offset leads to fainter X-ray emission. The X-ray constraints for hostless events are either too shallow or not consistent with the observed trend. Although this does not conclusively rule out that these hostless sGRBs could be mergers kicked out in the IGM, it does not offer observational support and leaves their nature undetermined. 

The main factors preserving the ambiguity in interpreting these events are \textit{i}) that the distance scale to the sGRB is not known and \textit{ii}) that the natal kick velocity and merger delay time are not known \textit{a priori}. Therefore, in order to disentangle between the faint host and large offset scenarios requires ...
- rapid AG spectroscopy
- KN detection
- GWs (Einstein telescope)




%Previous work in the literature \citep[see, e.g., ][]{Berger2010a,Tunnicliffe2014} has focused on the likelihood to detect faint galaxies at high-$z$, as opposed to the large probability of chance coincidence even in the event that a galaxy is detected. %For example, \citet{Berger2010a} found that galaxies with $r$\,$>$\,$26$ mag are consistent with the luminosity ($L$\,$\approx$\,$0.1$\,$-$\,$1$\,$L^*$) of typical sGRB hosts for $z$\,$>$\,$1.5$ (see also Figure \ref{fig: rband_vs_z}), and \citet{Tunnicliffe2014} concluded that faint, undetected hosts could exist at $z$\,$>$\,$1$. %In both cases, their findings are consistent with the observed luminosity of sGRB hosts at $z$\,$>$\,$1$ (Figure \ref{fig: rband_vs_z}).



==> O'Connor et al. Host Galaxies Paper/old_intro.tex <==

%Biases for using only optically localized GRBs: \\
%1) higher density \\
%2) lower redshift, calculate at what redshift does a balmer break fall in the r-band (need to emphasize most follow-up in the optical and say this is redshift at which balmer break affects optical observations \\
%3) intrinsic dust in host galaxy (dark GRBs) --> can exclude GRBs with small offsets from host galaxy due to high dust which can bias offset dist towards larger offsets and less dusty/star forming galaxies. e.g. 200522A where HST imaging was required to detect the afterglow conclusively.  \\
%See discussions in dark GRB papers of these biases.
%4)Kilonova bias (not sure if we want to include this) - if we just focus on events with redshifts and galaxies and bright optical KN we create a view of sGRBs associated to luminous KN which affects our understanding of the populations by selecting events with bright KN i.e., large KN ejecta.  \\
%\vspace{10mm}


Short duration gamma-ray bursts (sGRB) are bright, brief flashes of gamma-rays \citep[$<$\,$2$ s;][]{Chryssa93} created by the coalescence of two compact objects, either a binary neutron star system \citep[i.e., GW 170817;][]{Abbott2017, Goldstein2017, Savchenko2017} or a neutron star and a black hole \citep[BNS or NS-BH;][]{Eichler1989,Narayan1992}. Beginning in the era of the \textit{Neil Gehrels Swift Observatory} (hereafter \textit{Swift}; \citealt{Gehrels04}), sGRBs were, for the first time, localized to arcsecond accuracy based on the detection of their X-ray afterglows \citep{Burrows2005}. 
%To date, $\sim$\,$100$ sGRB have been localized in this way, but only $\sim$\,$40\%$ of these events have sub-arcsecond localization from the identification of their optical afterglows. 
These accurate (XRT and optical) localizations allowed for the identification of their host galaxies, and, in turn, their redshifts. 
Short GRBs have been associated to an eclectic distribution of galaxies, with a wide range in stellar mass \citep{Leibler2010} and star formation rate \citep{Berger2014}, as well as a mix of both early and late-type galaxies \citep{Fong2013}. 
These events are observed to occur at large physical offsets (up to $\sim$\,$75$ kpc) from the center of their host galaxies, and, therefore, potentially in tenuous (low density) environments \citep{Troja2008,FongBergerFox}. 


These factors have helped solidify sGRB as a unique class of transient, independent of long GRBs and their collapsar progenitors \citep{Hjorth2003,Hjorth2005}. However, our understanding of the environments of BNS mergers is still evolving, specifically regarding the $\sim$\,$20\%$ of events deemed hostless due to their lack of a coincident galaxy to deep limits ($\gtrsim$\,26 mag; \citealt{Berger2010a,FongBerger2013,Tunnicliffe2014}). 
Although there is no coincident galaxy, candidate hosts have been identified at offsets greater than $5\times$ the half-light radius $R_e$ of the galaxy \citep{FongBerger2013,Tunnicliffe2014}; localizing the sGRBs to well outside of the galaxy light.
These sGRBs are labeled as hostless, hereafter referred to as \textit{observationally} hostless, due to their lack of strong host galaxy association. 



The definition of an \textit{observationally} hostless burst does not specify a physical offset distance at which there is no strong association, but instead relies on probabilistic arguments \citep[e.g.,][]{Bloom2002,Bloom2007,Cobb2006,Levan2007,Cobb2008,Berger2010a}. The standard method for calculating the probability of chance coincidence, $P_{cc}$, uses the sky density of galaxies measured in deep optical and near-infrared (nIR) surveys \citep{Hogg1997,Beckwith2006,Metcalfe2006} to determine the probability of finding a random galaxy that is at least as bright within the localization region. 
Thus, bright, low-$z$ galaxies at significant offsets, such as $\gtrsim$\,$5R_e$ \citep{FongBerger2013}, can still be found to have a small probability of random alignment due to their lower number density on the sky.

These large offsets are expected in the kicked progenitor scenario, in which a large natal kick is imparted to the BNS system at formation, following mass ejection from the second supernova explosion \citep{Lyne1994,Hansen1997,Bloom1999,Fryer1999,Wex2000,Belczynski2006,Church2011,Behroozi2014}. Combined with the large merger delay times predicted for BNS systems, the natal kick may allow the BNS to escape its birth galaxy \citep{Zheng2007,Zemp2009,Behroozi2014}. 
However, in contrast to predictions for BNS natal kick velocities based on the observed distribution of pulsar velocities \citep{Lyne1994,Hansen1997,Hobbs2005}, \citet{Beniamini2016} and \citet{Beniamini2016p2} identified that $60-70\%$ of the Galactic BNS population likely received natal kicks on the order of $30$ km s$^{-1}$; too small to lead to significant offsets or escape their birth galaxies. 
In addition, \citet{BeniaminiPiran2019} demonstrated that $\gtrsim 40-60\%$ of Galactic BNS merge rapidly; in less than $1$\,$-$\,$2$ Gyr. 
These low kick velocities and short merger delay times observed in Galactic BNS systems, imply that a small fraction of BNS escape their birth galaxies; indicating a negligible population of \textit{physically} hostless sGRBs. 

In this work, we define a \textit{physically} hostless sGRB as having occurred in the intergalactic medium (IGM) outside of its birth galaxy's virial radius \citep{OConnor2020}. 
The distinction between \textit{observationally} and \textit{physically} hostless sGRBs is important. A physically hostless sGRB has escaped its birth galaxy, and at the time of merger is located in the IGM, which is the lowest density environment in the Universe \citep[making detection of an afterglow unlikely, e.g.,][]{Panaitescu2001,Salvaterra2010,Duque2019}. \citet{OConnor2020}  found that $\lesssim 16\%$ of sGRB have circumburst densities consistent with such large offsets (i.e., $<10^{-4}$ cm$^{-3}$). 
On the other hand, an observationally hostless sGRB may only appear to lack a putative host galaxy due either to 
\textit{i}) that the chance probability of association at the BNS merger radius, calculated using the sky density of galaxies \citep{Bloom2002}, is too large for a strong association with the true host galaxy or 
\textit{ii}) that the sGRB occurred in an undetected, faint host galaxy at intermediate to high redshifts (i.e., $z$\,$\gtrsim$\,$1$\,$-$\,$2$; 
\citealt{Berger2010a,Tunnicliffe2014,OConnor2020}). 
These are the two most likely explanations for observationally hostless sGRBs, given that the expected fraction of BNS escaping their host galaxies is likely small. Disentangling between these two scenarios is extremely difficult, and requires sensitive observations either with large-aperture ground-based instruments (e.g., Gemini, Keck) or space-based observatories (i.e, \textit{HST} or \textit{JWST}). 

While a bright galaxy is easily associated to a GRB, the association with a faint host galaxy relies on an accurate localization, as increasing the localization region leads to a higher probability of random sky alignment with an unrelated galaxy. 
It is for this reason that previous samples of sGRB hosts focused on the events with a sub-arcsecond localization \citep[e.g.,][]{FongBerger2013,Fong2013}.
However, focusing only on sGRB with detectable optical afterglows may bias the observed sample towards those occurring in higher density environments that produce bright afterglows \citep{Panaitescu2001,Salvaterra2010,Duque2019} or away from bursts occurring in dusty (star forming) environments, due to a small offset from the host's nucleus (requiring deep \textit{HST} nIR imaging and image subtraction for a solid identification, e.g., GRB 200522A; \citealt{Fong2021,OConnor2021}). In addition, those GRB with only an X-ray detection may be located at higher redshifts where either they are faint intrinsically or the 4000 \AA\,Balmer break reduces the observed flux at the wavelengths typically explored by ground-based follow-up (e.g., $r$-band for $z\gtrsim0.6$).

In this work, we targeted a sample of 31 sGRB that lacked a bright host galaxy with large-aperture instruments to search for faint, coincident galaxies. In order to offset any bias  against XRT localized events, we include 14 bursts with only an XRT position. While these bursts generally have poorly constrained offsets from their host galaxies, they contribute valuable information to the demographics of sGRB galaxies in terms of redshift, stellar mass, star formation rate, and galaxy type \citep[e.g.,][]{Gehrels2005,Bloom2006}.
This has implications for the follow-up of electromagnetic (EM) counterparts to gravitational waves from BNS mergers as the quick localization of the EM counterpart depends on inferences (such as, e.g., stellar mass and star formation rate) from the known population of sGRB \citep[e.g.,][]{Nissanke2013,Gehrels2016,Coulter2017,Arcavi2017,Artale2020,Ducoin2020} and on targeted searches using catalogs of nearby galaxies \citep[e.g.,][]{White2011,Dalya2016,Cook2019}.

The paper is outlined as follows. In \S \ref{sec: observations}, we define our sample selection criteria, and the optical/nIR imaging analysis techniques used in this work. In \S \ref{sec: methods}, we describe the methods employed to detect, localize, and compute photometry of the host galaxies, as well as the probabilistic criteria used for host assignment. The results are presented in \S \ref{sec: Results} (see also Appendix \ref{sec: appendixsampleanalysis}) and we discuss the demographics of sGRB offsets, host galaxies, and environments in \S \ref{sec: host_demo_intro}. We present a discussion of these results in \S \ref{sec: discussion} and conclude in \S \ref{sec: conclusions}.

We adopt the standard $\Lambda$-CDM cosmology with parameters $H_0=67.4$, $\Omega_M=0.315$, and $\Omega_\Lambda=0.685$ \citep{Planck2018}. 
 All confidence intervals are at the $1\sigma$ level and upper limits at the $3\sigma$ level, unless otherwise stated. 
 All reported magnitudes are in the AB system, and are corrected for Galactic extinction \citep{Schlafly2011}.
 Throughout the paper we adopt the convention $F_\nu\propto t^{-\alpha}\nu^{-\beta}$.




==> O'Connor et al. Host Galaxies Paper/old_xray_table.tex <==
\begin{table*}
 	\centering
 	\caption{Short GRB X-ray afterglow properties. The parameters $t_o$, $F_{X,o}$, and $n_\textrm{min}$ are defined as in \citet{OConnor2020}. $\alpha_X$ and $\beta_X$ are the temporal and spectral indices of the early X-ray afterglow. 
 	\brendan{I do not like adding $\alpha$ or $\beta$ because for cases like 180618A where the best fit model has 3 breaks it is not clear which our slope refers to! I have tried to make it the value at the time we are taking the data point for... also alpha/beta are not needed to compute the density...}
 	\textcolor{red}{check that all time and flux here agree with my other paper. And then re-check density if they do not...}
 	}
 	\label{tab: XrayAGprop}
 	\begin{tabular}{lccccc}
    \hline
       \hline
       \\[-2.5mm]
   \textbf{GRB} & \textbf{$t_o$} & \textbf{$\alpha_X$} & \textbf{$\beta_X$}  & \textbf{$F_{X,o}$} & \textbf{$n_\textrm{min}$} \\
   & \textbf{(s)} & & & \textbf{($10^{-11}$ erg cm$^{-2}$ s$^{-1}$)} & \textbf{(cm$^{-3}$)}\\
    \hline
 091109B & $160^{+120}_{-70}$ & $0.7\pm0.1$ & $0.9^{+0.5}_{-0.2}$ & $1.0\pm0.2$ & \\[0.9mm]
 101224A & $630^{+780}_{-540}$ & -- & -- & $0.02\pm0.01$ & $3.6\times 10^{-6}$ \\[0.9mm]
 110112A & $190\pm100$  & $1.06\pm0.10$ & $1.3^{+0.5}_{-0.4}$ & $1.4\pm0.4$ & $1.4\times 10^{-3}$ \\[0.9mm]
110402A$^a$  & $590\pm40$ & $0.4\pm0.2$ & $0.89\pm0.25$ & $1.0\pm0.2$ & $4.0\times10^{-4}$ \\[0.9mm]
120305A  & $350^{+250}_{-90}$  & $1.6\pm0.5$ & $1.9\pm0.7$ & $1.1\pm0.2$ & $2.0\times 10^{-5}$ \\[0.9mm]
 120630A & $175_{-80}^{+120}$ & $1.6\pm0.5$ & $0.7^{+0.6}_{-0.3}$ & $0.48\pm0.11$ & $9.0\times 10^{-5}$\\[0.9mm]
 130822A & -- & $\sim$\,$8.0$ & $1.1^{+1.8}_{-0.9}$ & -- & -- \\[0.9mm]
 130912A & $160\pm20$ & $1.2\pm0.08$ & $0.5\pm0.15$ & $24\pm5$ & $2.1\times 10^{-3}$ \\[0.9mm]
 131004A & $120^{+40}_{-50}$ & $0.96\pm0.07$ & $0.97\pm0.18$ & $3.8\pm0.8$ & $1.5\times10^{-3}$ \\[0.9mm]
140129B  & $330\pm10$  & $1.2\pm0.1$ & $1.0\pm0.2$ & $5.6\pm1.3$ & $1.0\times 10^{-3}$ \\[0.9mm]
 140516A & $200^{+2400}_{-110}$ & -- & $0.4^{+1.0}_{-0.4}$ & $0.06\pm0.02$ & $9.0\times 10^{-5}$ \\[0.9mm]
140622A  & $300^{+1100}_{-100}$ & $3.0\pm1.0$ & $0.6^{+0.7}_{-0.4}$ & $0.04\pm0.01$ & $1.8\times 10^{-5}$ \\[0.9mm]
 140930B & $187\pm4$  & $1.17\pm0.12$ & $0.7\pm0.2$ & $40\pm5$ & $1.4\times 10^{-3}$ \\[0.9mm]
 150423A & $110\pm30$ & $1.01\pm0.10$ & $0.51^{+0.36}_{-0.25}$ & $1.6\pm0.4$ & $2.6\times 10^{-4}$ \\[0.9mm]
 150831A & $240^{+90}_{-40}$ & $1.1\pm0.2$ & $0.8^{+0.5}_{-0.4}$ & $1.5\pm0.4$ & $2.4\times 10^{-5}$ \\[0.9mm]
 151229A & $76\pm4$ & $0.54\pm0.12$ & $1.03\pm0.14$ & $33\pm4$ & $1.2\times 10^{-1}$ \\[0.9mm]
 160408A & $300\pm20$ & $1.6\pm0.4$ & $1.0\pm0.4$ & $3.2\pm0.7$ & $1.8\times 10^{-4}$ \\[0.9mm]
 160410A$^a$ & $360\pm8$ & $1.2\pm0.2$ & $0.33\pm0.10$ & $8.0\pm2.0$ & $2.6\times10^{-3}$ \\[0.9mm]
 160525B & $73\pm3$  & $1.4\pm0.1$ & $0.95\pm0.25$ & $10.5\pm3.0$ & $6.6\times 10^{-3}$ \\[0.9mm]
 160601A & $270^{+420}_{-190}$ & $0.44\pm0.15$ & $1.0^{+0.8}_{-0.5}$ & $0.10\pm0.02$ & $8.2\times10^{-6}$ \\[0.9mm]
160927A  & $130^{+30}_{-50}$  & $1.02\pm0.09$  & $0.65^{+0.30}_{-0.15}$ &$1.9\pm0.4$ & $1.1\times10^{-4}$ \\[0.9mm]
 170127B & $130^{+50}_{-30}$ & $1.9\pm0.7$ & $0.6^{+0.4}_{-0.2}$ & $6.0\pm1.0$ & $7.3\times 10^{-4}$ \\[0.9mm]
  170428A & $800^{+150}_{-100}$ & $1.0\pm0.2$ & $2.0^{+1.3}_{-1.0}$ & $0.25\pm0.06$ & $1.6\times 10^{-5} $\\[0.9mm]
 170728A & $250^{+70}_{-50}$ & $0.90\pm0.10$ & $1.1^{+0.3}_{-0.1}$ & $1.0\pm0.2$ &  $1.2\times 10^{-4}$ \\[0.9mm]
 170728B$^a$ & $460\pm2$  & $0.6\pm0.1$ & $1.0\pm0.1$ & $37\pm7$ & $7.5\times 10^{-4}$ \\[0.9mm]
  171007A$^a$ &  $370^{+1500}_{-130}$ & $0.7^{+0.2}_{-0.7}$  & $0.36^{+0.49}_{-0.25}$ & $0.17\pm0.03$ & $8.0\times10^{-7}$ \\[0.9mm]
 180618A$^a$ & $69.1\pm0.6$  & $0.82\pm0.15$ & $0.88\pm0.08$ & $130\pm20$ & \textcolor{red}{XX} \\[0.9mm]
 180727A & $230^{+70}_{-50}$ & $1.0\pm0.4$ & $0.8\pm0.4$ & $1.5\pm0.3$ & $3.0\times 10^{-5}$ \\[0.9mm]
 180805B$^a$ & $1300^{+90}_{-130}$ & $1.04\pm0.16$ & $1.1\pm0.5$ & $0.25\pm0.07$ & $3.0\times 10^{-6}$ \\[0.9mm]
 191031D & $120\pm20$ & $2.0\pm0.2$  & $0.95^{+0.31}_{-0.16}$ & $2.9\pm0.7$ & \textcolor{orange}{XX} \\[0.9mm]
 200411A & $280^{+90}_{-80}$ & $0.9\pm0.2$ & $0.7\pm0.2$  & $1.0\pm0.2$ & $2.3\times10^{-4}$ \\[0.9mm]
     \hline
    \end{tabular}
\begin{flushleft}
    \quad \footnotesize{$^a$ Short GRB with extended emission.} \\
    \quad \footnotesize{$^b$ The early X-ray lightcurve of this GRB does not fit the criteria outlined by \citet{OConnor2020}.} \\
\end{flushleft}
\end{table*}


==> O'Connor et al. Host Galaxies Paper/table_test.tex <==
\begin{table*}
 	\centering
 	\caption{Log of short GRB host galaxy observations. \brendan{Make another table for the spectroscopic observations?}
 	}
 	\label{tab: observations}
 	\begin{tabular}{lccccccccccc}
    \hline
       \hline 
       \\[-2.5mm]
   \textbf{GRB} & \textbf{$T_{90}^c$} & \textbf{RA} & \textbf{Dec} &\textbf{Obs. Date}  &   \textbf{Telescope} & \textbf{Instrument} & \textbf{Filter} & \textbf{Exp.} &  \textbf{AG Image}$^{b}$ & \textbf{AB Mag} &\textbf{$A_\lambda$}  \\
   & \textbf{(s)} &  \textbf{(J2000)} & \textbf{(J2000)} & \textbf{(UT)} & & & & \textbf{(s)} & &   & \textbf{(mag)} \\
    \hline
%    090621B &  0.14 &  20:53:53.17 &  69:01:41.4	 &  06-14-2014 3:27:41 & LDT & LMI  & \textit{r} & 3780  & ... & 1.37 \\
%    ... &  ... & ... & ... &  10-25-2014 06:10:33 & Keck & LRIS  & \textit{G} & 2700  & ...  & ... \\
%    ... &  ... & ... & ...  & 10-25-2014 06:16:45  & Keck  & LRIS & \textit{R} & 2000  & ...  & ...   \\
%    \hline
   091109B & 0.3 & 07:30:56.61 & -54:05:22.85 & 11-10-2009   & VLT & FORS2  & \textit{R}  & 3600 & Y &   0.45 \\
   ... & ... & ... & ... & 02-26-2012 & \textit{HST} & WFC3 & \textit{F160W} & 5600 & ... &   ...\\
   ... & ... & ... & ... & 11-01-2016  & \textit{HST} & WFC3 & \textit{F110W} & 5600 & ... &   ...\\
   \hline
   110112A & 0.5 & 21:59:43.85 & 26:27:23.9 &  01-12-2011  & WHT & ACAM &  \textit{i} & 900 & Y & 0.16\\
      ... & ... & ... & ... & 10-13-2016   & \textit{HST} & WFC3 & \textit{F110W} & 5200 & ... &   ...\\
   \hline
  110402A$^{a}$  & 60.9 & 21:59:43.85 & 26:27:23.9 & \textcolor{red}{xxx} & \textit{Swift} & UVOT & \textcolor{red}{xxx} & \textcolor{red}{xxx} &  Y & 0.05\\
   ... & ... & ... & ... & 08-03-2020  & Gemini & GMOS-N & \textit{r} & 900 & ... &  ...  \\
     ... & ... & ... & ... & 05-05-2021  & LDT & LMI & \textit{i} & 1500 & ... &  ...  \\
  ... & ... & ... & ... & 05-06-2021  & LDT & LMI & \textit{z} & \textcolor{red}{xxx} & ... &  ...  \\
    \hline
  120305A  & 0.1 & 03:10:08.68 & 28:29:31.0 & 03-06-2014	  & LDT  & LMI & \textit{r} & 2700 & ... & 1.15 \\
  ... & ... & ... & ... & 10-25-2014	&   Keck& LRIS&\textit{G}& 3000 & ... & ... \\
    ... & ... & ... & ... & 10-25-2014	&  Keck& LRIS&\textit{R} & 2750 & ... & ... \\
  \hline
  120630A  & 0.6 & 23:29:11.07 & 42:33:20.3 & 07-01-2012   & Gemini  & GMOS-N & \textit{r} & 500 & ... &  0.29 \\
    ... & ... & ... & ... &07-01-2012& Gemini & GMOS-N & \textit{i} & 500 & ... &  ... \\
      ... & ... & ... & ... &07-01-2012 & Gemini & GMOS-N & \textit{z} & 500 & ... &  ... \\
  ... & ... & ... & ... & 09-05-2014  & LDT & LMI & \textit{r} & 700 & ... &  ... \\
 ... & ... & ... & ... &09-05-2014 & LDT & LMI & \textit{i} & 400 & ... &  ... \\
  ... & ... & ... & ... &2014-09-05	 & LDT & LMI & \textit{z} & 800 & ... &  ... \\
  ... & ... & ... & ... &10-25-2014 & Keck & LRIS & \textit{R} & 3300 & ... &  ... \\
    ... & ... & ... & ... &10-25-2014 & Keck & LRIS & \textit{G} & 3600 & ... &  ... \\
 %  \hline
 %    \textcolor{magenta}{121226A} &  & & & & & & & & & \\
 %  ... & ... & ... & ... & &  &  &  & & ... & ... \\
  \hline
  130822A  & 0.04 & 01:51:41.27 & -03:12:31.7 & 08-23-2013	 & Gemini & GMOS-N & \textit{i} & 600 & ... &  0.08 \\
  ...  & ... & ... & ... & 10-25-2014 & Keck & LRIS & \textit{G} & 3000 & ... & ... \\
   ...  & ... & ... & ... & 10-25-2014	 & Keck & LRIS & \textit{R} & 2750 & ... & ... \\
  \hline
  130912A  & 0.28 & 03:10:22.23 & 13:59:48.7 & 09-13-2013  & WHT & ACAM & \textit{i} & 900 & Y & 0.76 \\
  ...  & ... & ... & ... & 02-25-2014  & LDT & LMI & \textit{r} & 2700 & ... & ... \\
  ...  & ... & ... & ... &10-25-2014   & Keck & LRIS &  \textit{G} & 2400 & ... & ... \\
 ...  & ... & ... & ... & 10-25-2014  & Keck & LRIS & \textit{R}  & 2750  & ... & ... \\
  ...  & ... & ... & ... & 01-09-2017  & \textit{HST} & WFC3 & \textit{F110W} & 5200 & ... & ... \\
   \hline
    131004A   & 1.54 & 19:44:27.08& -02:57:30.2 & \textcolor{red}{xxx} & \textit{Swift} & UVOT & \textit{wh} & \textcolor{red}{xxx} & Y & 0.76 \\
      ...& ... &...& ...& \textcolor{red}{xxx}  & Keck & MOSFIRE & \textit{$K_s$} & \textcolor{red}{xxx}  & ... &  \\
     ...  & ... & ... & ... & 10-11-2016 & \textit{HST} & WFC3 & \textit{F110W} & 5212 & ... & 0.77 \\
  \hline
  140930B  & 0.84 &  00:25:23.4 &24:17:41.7 &09-30-2014	& WHT & ACAM & \textit{r} & 3800 & Y & 0.08 \\ 
     ...  & ... & ... & ... & & LDT & &  & & ... & ... \\
   ...  & ... & ... & ... & 08-01-2020 & Gemini & GMOS-N &  \textit{r}& 1650 & ... & ... \\
  \hline
  150423A  & 0.08 & 14:46:18.86 & 12:17:00.70 &  04-23-2015 08:02:19 & VLT & FORS2 & \textit{R} & 300 & Y & 0.08 \\
    ...  & ... & ... & ... & 02-03-2017  & \textit{HST} & WFC3 & \textit{F110W} & 5200 & ... & ... \\
  \hline
  151229A  & 1.44 &21:57:28.78& 	-20:43:55.2 & 03-08-2019 & LDT & LMI & \textit{r}&1200 & ... & 0.07 \\
  ...& ... &...& ...& 07-30-2019   & Gemini &GMOS-S & \textit{z}&1920 & ... &  \\
  ...& ... &...& ...& 10-15-2019   & Keck & MOSFIRE & \textit{Y} & 1340 & ... &  \\
  ...& ... &...& ...& 08-11-2020   & Gemini & GMOS-N & \textit{r}&2250 & ... & ...  \\
  ...& ... &...& ...& 06-16-2021  & LDT & LMI & \textit{i}& 900 & ... & ...  \\
  \hline
  160601A  & 0.12 & 15:39:43.97 & 64:32:30.5 & 06-02-2016  &  Gemini & GMOS-N & \textit{r} & 900 & Y & 0.07 \\
   ... & ... & ... & ... & 06-03-2016  & LDT  & LMI & \textit{r} & 720 & ... & ...\\
 ... & ... & ... & ... & 08-01-2020	 & Gemini & GMOS-N & \textit{r} & 1800 & ... & ... \\
  \hline
  160927A  & 0.48 & 17:04:58.22 & 17:19:54.9 & 09-28-2016  & GTC & OSIRIS & \textit{r} & 1915 & Y & 0.21 \\
   ... & ... & ... & ... & 02-23-2017   & GTC   & OSIRIS  &\textit{r}  & 1200 & ... & ... \\
   ... & ... & ... & ... & 05-20-2018    & LDT  &  LMI & \textit{r} & 300 & ... & ... \\
   ... & ... & ... & ... & 08-01-2020    & Gemini & GMOS-N & \textit{i} & 720 & ... & ... \\
  % ... & ... & ... & ... & &  &  &  & & ... & ... \\
  \hline
   170127B & 0.5  &01:19:54.47 &-30:21:28.6 & 2018-01-27 & Gemini & GMOS-S & \textit{g} & 1800 &... & 0.06 \\
    ... & ... & ... & ... & 2018-10-06 & Keck & LRIS &\textit{G}  & 2520 & ... & ... \\
    ... & ... & ... & ... & 2018-10-06  & Keck & LRIS &\textit{R}  & 1720 & ... & ... \\
    ... & ... & ... & ... & 2019-09-04  & Keck & LRIS &\textit{G}  & 1920 & ... & ... \\
    ... & ... & ... & ... & 2019-09-04 & Keck & LRIS &\textit{I}  & 1600 & ... & ... \\
    ... & ... & ... & ... & 2019-10-15  & Keck & MOSFIRE &\textit{J}  & 2010 & ... & ... \\
    ... & ... & ... & ... & 01-30-2021 & Gemini & GMOS-S &\textit{z}  & 1440 & ... & ... \\
    \hline
   171007A$^a$ & 105 &09:02:24.14 & 42:49:08.8 & 01-09-2020  & LDT & LMI & \textit{r}  & 1200 & ... &  0.06\\
    ... & ... & ... & ... & 02-01-2021  & Gemini  & GMOS-N  & \textit{i}  & 1440 & ... & ... \\
      \hline
 170728A  & 1.3  &03:55:33.17 & 12:10:54.7 & \textcolor{red}{xxx} & \textit{Swift} & UVOT & & & Y & 0.65 \\
    ... & ... & ... & ... & 01-14-2018  & Keck & LRIS  & \textit{G}  & 1380 & ... & ... \\
    ... & ... & ... & ... & 01-14-2018 & Keck & LRIS  & \textit{R}  & 1380 & ... & ... \\
    ... & ... & ... & ... &  \textcolor{red}{xxx} & LDT & LMI  &   \textit{r} & & ... & ... \\
 %       \hline
 % \textcolor{magenta}{180618A$^a$} &  & & & & & & & & & \\
 %  ... & ... & ... & ... & &  &  &  & & ... & ... \\
         \hline
   191031D & 0.3 &18:53:09.57 &47:38:38.8 & 11-02-2019  & Gemini & GMOS-N & \textit{r} & 720 & ... & 0.2 \\
    ... & ... & ... & ... & 11-03-2019 & LDT  & LMI  & \textit{g}  &1200& ... & ... \\
    ... & ... & ... & ... & 11-03-2019 & Gemini  & GMOS-N &  \textit{i} & 355 & ... & ... \\
    ... & ... & ... & ... & \textcolor{red}{xxx} & LDT & LMI  &   \textit{g} & & ... & ... \\
    ... & ... & ... & ... &\textcolor{red}{xxx} & LDT & LMI  &   \textit{i} & & ... & ... \\
    ... & ... & ... & ... &\textcolor{red}{xxx} & LDT & LMI  &  \textit{z} & & ... & ... \\
    ... & ... & ... & ... &\textcolor{red}{xxx} & LDT & LMI  &  \textit{Y} & & ... & ... \\
\hline
  200411A  & 0.33  &03:10:39.39	 & -52:19:03.4 &01-25-21 & Gemini & GMOS-S & \textit{r} & 1800 & ... & 0.06\\
 % \hline
 %   & & & & & & & & & &  \\
 %   & & & & & & & & & &  \\
 %   & & & & & & & & & &  \\
 %   & & & & & & & & & & \\
 %   & & & & & & & & & & \\
 %   & & & & & & & & & & \\
     \hline
    \end{tabular}
\begin{flushleft}
    \quad \footnotesize{$^a$ Short GRB with extended emission.} \\
    \quad \footnotesize{$^b$ Afterglow image used for relative alignment.}\\
    \quad \footnotesize {$^c$ $T_{90}$ values were retrieved from the \textit{Swift} BAT GRB catalog \citep{Lien2016}.}\\
   % \quad \footnotesize {$^d$ Galactic extinction in the direction of the burst \citep{Schlafly2011}.}\\
\end{flushleft}
\end{table*}

==> new_disc_tes.tex <==
\nora{
2) There is a lingering ambiguity in the origin of hostless events. For instance, 
the sample of Berger lies close to nearby galaxies and could be either highly offset or high redshift. This works finds a large fraction of hostless events NOT associated to any nearby galaxy, but either faint or undetected hosts. 
Therefore we can say that XX per cent of hostless are likely high-z events.
3) We also examine the sample of hostless events that do lie close to a nearby galaxy, and in particular use their high-energy properties to probe their environment.  We do find a trend correlating the brightness of the X-ray afterglow with the GRB location, being large offset events also X-ray faint. 
We note that X-ray constraints of hostless events are either too shallow or not consistent with the observed trend.  Although this does not conclusively rule out that these hostless GRBs could be mergers kicked out in the IGM, it does not offer observational support and leave their nature undetermined. 
The most critical observational tests would be: 1) rapid afterglow spectroscopy (16410A), to
determine the distance scale directly from the afterglow. 2) rapid and deep X-ray observations, capable of probing X-ray fluxes of 1e-16 within 12 hrs since the GRB. 
This is ATHENA but it is not expected to fly for the next 12 years! 3) detect a kilonova which would provide an indirect evidence of a low-z due to their maximum peak luminosity (Chase et al...)
}


We emphasize that there is a lingering ambiguity as to the origin of hostless short GRBs. For instance, the hostless sGRBs presented by \citet{Berger2010a} are located at a significant offset ($30$\,$-$\,$75$ kpc) from bright low-$z$ ($z<0.5$) galaxies. However, despite their brightness, the probability of chance coincidence is $\gtrsim 10\%$. Therefore, it is not clear whether these sGRBs are truly associated to these low-$z$ galaxies, or whether they reside in faint, undetected host galaxies. 

In this work, we have tripled the number of observationally hostless sGRBs (from 7 to 20 events). We instead uncovered a population of 9 observationally hostless sGRBs (see \S \ref{sec: hostlum}) without any nearby (low-$z$) candidate host galaxy. As such, these events are more likely to have exploded in faint $r\gtrsim 24.5$ mag galaxies, which are consistent with $0.1-1.0L^*$ galaxies at $z>1$. Therefore, we set a lower limit of $>45\%$ to the fraction of hostless sGRBs at high-$z$.

A larger population of sGRBs at $z$\,$>$\,$1$ implies a steep DTD with an increased fraction of events with short delay times, as deduced based on Galactic BNS systems \citep[][]{BeniaminiPiran2019}. We note, however, that an alternative explanation is that these are due to a population of low luminosity ($<$\,$0.1 L^*$) galaxies hosting sGRBs at $z$\,$<$\,$1$, although this at tension with the population of well-determined sGRB hosts ($0.1$\,$-$\,$1 L^*$; \citealt{Berger2010a}) and with predictions from population synthesis modeling, which find that BNS systems preferentially form in the most massive (brightest) galaxies \citep{Behroozi2014,Mapelli2018,Artale2019,Artale2020,Adhikari2020,Mandhai2021,Chu2022}. 

We further explored the sample of observationally hostless events that lie close to low-$z$ galaxies. We exploited their high-energy properties to probe their environments (\S \ref{sec: environment}). Figure \ref{fig: fluxfluence_vs_offset} shows a weak correlation between the brightness of the X-ray afterglow with the sGRB location, such that a larger offset leads to fainter X-ray emission. The X-ray constraints for hostless events are either too shallow or not consistent with the observed trend. Although this does not conclusively rule out that these hostless sGRBs could be mergers kicked out in the IGM, it does not offer observational support and leaves their nature undetermined. 

The main factors preserving the ambiguity in interpreting these events are \textit{i}) that the distance scale to the sGRB is not known and \textit{ii}) that the natal kick velocity and merger delay time are not known \textit{a priori}. Therefore, in order to disentangle between the faint host and large offset scenarios requires ...
- rapid AG spectroscopy
- KN detection
- GWs (Einstein telescope)




%Previous work in the literature \citep[see, e.g., ][]{Berger2010a,Tunnicliffe2014} has focused on the likelihood to detect faint galaxies at high-$z$, as opposed to the large probability of chance coincidence even in the event that a galaxy is detected. %For example, \citet{Berger2010a} found that galaxies with $r$\,$>$\,$26$ mag are consistent with the luminosity ($L$\,$\approx$\,$0.1$\,$-$\,$1$\,$L^*$) of typical sGRB hosts for $z$\,$>$\,$1.5$ (see also Figure \ref{fig: rband_vs_z}), and \citet{Tunnicliffe2014} concluded that faint, undetected hosts could exist at $z$\,$>$\,$1$. %In both cases, their findings are consistent with the observed luminosity of sGRB hosts at $z$\,$>$\,$1$ (Figure \ref{fig: rband_vs_z}).



==> old_intro.tex <==

%Biases for using only optically localized GRBs: \\
%1) higher density \\
%2) lower redshift, calculate at what redshift does a balmer break fall in the r-band (need to emphasize most follow-up in the optical and say this is redshift at which balmer break affects optical observations \\
%3) intrinsic dust in host galaxy (dark GRBs) --> can exclude GRBs with small offsets from host galaxy due to high dust which can bias offset dist towards larger offsets and less dusty/star forming galaxies. e.g. 200522A where HST imaging was required to detect the afterglow conclusively.  \\
%See discussions in dark GRB papers of these biases.
%4)Kilonova bias (not sure if we want to include this) - if we just focus on events with redshifts and galaxies and bright optical KN we create a view of sGRBs associated to luminous KN which affects our understanding of the populations by selecting events with bright KN i.e., large KN ejecta.  \\
%\vspace{10mm}


Short duration gamma-ray bursts (sGRB) are bright, brief flashes of gamma-rays \citep[$<$\,$2$ s;][]{Chryssa93} created by the coalescence of two compact objects, either a binary neutron star system \citep[i.e., GW 170817;][]{Abbott2017, Goldstein2017, Savchenko2017} or a neutron star and a black hole \citep[BNS or NS-BH;][]{Eichler1989,Narayan1992}. Beginning in the era of the \textit{Neil Gehrels Swift Observatory} (hereafter \textit{Swift}; \citealt{Gehrels04}), sGRBs were, for the first time, localized to arcsecond accuracy based on the detection of their X-ray afterglows \citep{Burrows2005}. 
%To date, $\sim$\,$100$ sGRB have been localized in this way, but only $\sim$\,$40\%$ of these events have sub-arcsecond localization from the identification of their optical afterglows. 
These accurate (XRT and optical) localizations allowed for the identification of their host galaxies, and, in turn, their redshifts. 
Short GRBs have been associated to an eclectic distribution of galaxies, with a wide range in stellar mass \citep{Leibler2010} and star formation rate \citep{Berger2014}, as well as a mix of both early and late-type galaxies \citep{Fong2013}. 
These events are observed to occur at large physical offsets (up to $\sim$\,$75$ kpc) from the center of their host galaxies, and, therefore, potentially in tenuous (low density) environments \citep{Troja2008,FongBergerFox}. 


These factors have helped solidify sGRB as a unique class of transient, independent of long GRBs and their collapsar progenitors \citep{Hjorth2003,Hjorth2005}. However, our understanding of the environments of BNS mergers is still evolving, specifically regarding the $\sim$\,$20\%$ of events deemed hostless due to their lack of a coincident galaxy to deep limits ($\gtrsim$\,26 mag; \citealt{Berger2010a,FongBerger2013,Tunnicliffe2014}). 
Although there is no coincident galaxy, candidate hosts have been identified at offsets greater than $5\times$ the half-light radius $R_e$ of the galaxy \citep{FongBerger2013,Tunnicliffe2014}; localizing the sGRBs to well outside of the galaxy light.
These sGRBs are labeled as hostless, hereafter referred to as \textit{observationally} hostless, due to their lack of strong host galaxy association. 



The definition of an \textit{observationally} hostless burst does not specify a physical offset distance at which there is no strong association, but instead relies on probabilistic arguments \citep[e.g.,][]{Bloom2002,Bloom2007,Cobb2006,Levan2007,Cobb2008,Berger2010a}. The standard method for calculating the probability of chance coincidence, $P_{cc}$, uses the sky density of galaxies measured in deep optical and near-infrared (nIR) surveys \citep{Hogg1997,Beckwith2006,Metcalfe2006} to determine the probability of finding a random galaxy that is at least as bright within the localization region. 
Thus, bright, low-$z$ galaxies at significant offsets, such as $\gtrsim$\,$5R_e$ \citep{FongBerger2013}, can still be found to have a small probability of random alignment due to their lower number density on the sky.

These large offsets are expected in the kicked progenitor scenario, in which a large natal kick is imparted to the BNS system at formation, following mass ejection from the second supernova explosion \citep{Lyne1994,Hansen1997,Bloom1999,Fryer1999,Wex2000,Belczynski2006,Church2011,Behroozi2014}. Combined with the large merger delay times predicted for BNS systems, the natal kick may allow the BNS to escape its birth galaxy \citep{Zheng2007,Zemp2009,Behroozi2014}. 
However, in contrast to predictions for BNS natal kick velocities based on the observed distribution of pulsar velocities \citep{Lyne1994,Hansen1997,Hobbs2005}, \citet{Beniamini2016} and \citet{Beniamini2016p2} identified that $60-70\%$ of the Galactic BNS population likely received natal kicks on the order of $30$ km s$^{-1}$; too small to lead to significant offsets or escape their birth galaxies. 
In addition, \citet{BeniaminiPiran2019} demonstrated that $\gtrsim 40-60\%$ of Galactic BNS merge rapidly; in less than $1$\,$-$\,$2$ Gyr. 
These low kick velocities and short merger delay times observed in Galactic BNS systems, imply that a small fraction of BNS escape their birth galaxies; indicating a negligible population of \textit{physically} hostless sGRBs. 

In this work, we define a \textit{physically} hostless sGRB as having occurred in the intergalactic medium (IGM) outside of its birth galaxy's virial radius \citep{OConnor2020}. 
The distinction between \textit{observationally} and \textit{physically} hostless sGRBs is important. A physically hostless sGRB has escaped its birth galaxy, and at the time of merger is located in the IGM, which is the lowest density environment in the Universe \citep[making detection of an afterglow unlikely, e.g.,][]{Panaitescu2001,Salvaterra2010,Duque2019}. \citet{OConnor2020}  found that $\lesssim 16\%$ of sGRB have circumburst densities consistent with such large offsets (i.e., $<10^{-4}$ cm$^{-3}$). 
On the other hand, an observationally hostless sGRB may only appear to lack a putative host galaxy due either to 
\textit{i}) that the chance probability of association at the BNS merger radius, calculated using the sky density of galaxies \citep{Bloom2002}, is too large for a strong association with the true host galaxy or 
\textit{ii}) that the sGRB occurred in an undetected, faint host galaxy at intermediate to high redshifts (i.e., $z$\,$\gtrsim$\,$1$\,$-$\,$2$; 
\citealt{Berger2010a,Tunnicliffe2014,OConnor2020}). 
These are the two most likely explanations for observationally hostless sGRBs, given that the expected fraction of BNS escaping their host galaxies is likely small. Disentangling between these two scenarios is extremely difficult, and requires sensitive observations either with large-aperture ground-based instruments (e.g., Gemini, Keck) or space-based observatories (i.e, \textit{HST} or \textit{JWST}). 

While a bright galaxy is easily associated to a GRB, the association with a faint host galaxy relies on an accurate localization, as increasing the localization region leads to a higher probability of random sky alignment with an unrelated galaxy. 
It is for this reason that previous samples of sGRB hosts focused on the events with a sub-arcsecond localization \citep[e.g.,][]{FongBerger2013,Fong2013}.
However, focusing only on sGRB with detectable optical afterglows may bias the observed sample towards those occurring in higher density environments that produce bright afterglows \citep{Panaitescu2001,Salvaterra2010,Duque2019} or away from bursts occurring in dusty (star forming) environments, due to a small offset from the host's nucleus (requiring deep \textit{HST} nIR imaging and image subtraction for a solid identification, e.g., GRB 200522A; \citealt{Fong2021,OConnor2021}). In addition, those GRB with only an X-ray detection may be located at higher redshifts where either they are faint intrinsically or the 4000 \AA\,Balmer break reduces the observed flux at the wavelengths typically explored by ground-based follow-up (e.g., $r$-band for $z\gtrsim0.6$).

In this work, we targeted a sample of 31 sGRB that lacked a bright host galaxy with large-aperture instruments to search for faint, coincident galaxies. In order to offset any bias  against XRT localized events, we include 14 bursts with only an XRT position. While these bursts generally have poorly constrained offsets from their host galaxies, they contribute valuable information to the demographics of sGRB galaxies in terms of redshift, stellar mass, star formation rate, and galaxy type \citep[e.g.,][]{Gehrels2005,Bloom2006}.
This has implications for the follow-up of electromagnetic (EM) counterparts to gravitational waves from BNS mergers as the quick localization of the EM counterpart depends on inferences (such as, e.g., stellar mass and star formation rate) from the known population of sGRB \citep[e.g.,][]{Nissanke2013,Gehrels2016,Coulter2017,Arcavi2017,Artale2020,Ducoin2020} and on targeted searches using catalogs of nearby galaxies \citep[e.g.,][]{White2011,Dalya2016,Cook2019}.

The paper is outlined as follows. In \S \ref{sec: observations}, we define our sample selection criteria, and the optical/nIR imaging analysis techniques used in this work. In \S \ref{sec: methods}, we describe the methods employed to detect, localize, and compute photometry of the host galaxies, as well as the probabilistic criteria used for host assignment. The results are presented in \S \ref{sec: Results} (see also Appendix \ref{sec: appendixsampleanalysis}) and we discuss the demographics of sGRB offsets, host galaxies, and environments in \S \ref{sec: host_demo_intro}. We present a discussion of these results in \S \ref{sec: discussion} and conclude in \S \ref{sec: conclusions}.

We adopt the standard $\Lambda$-CDM cosmology with parameters $H_0=67.4$, $\Omega_M=0.315$, and $\Omega_\Lambda=0.685$ \citep{Planck2018}. 
 All confidence intervals are at the $1\sigma$ level and upper limits at the $3\sigma$ level, unless otherwise stated. 
 All reported magnitudes are in the AB system, and are corrected for Galactic extinction \citep{Schlafly2011}.
 Throughout the paper we adopt the convention $F_\nu\propto t^{-\alpha}\nu^{-\beta}$.




==> old_xray_table.tex <==
\begin{table*}
 	\centering
 	\caption{Short GRB X-ray afterglow properties. The parameters $t_o$, $F_{X,o}$, and $n_\textrm{min}$ are defined as in \citet{OConnor2020}. $\alpha_X$ and $\beta_X$ are the temporal and spectral indices of the early X-ray afterglow. 
 	\brendan{I do not like adding $\alpha$ or $\beta$ because for cases like 180618A where the best fit model has 3 breaks it is not clear which our slope refers to! I have tried to make it the value at the time we are taking the data point for... also alpha/beta are not needed to compute the density...}
 	\textcolor{red}{check that all time and flux here agree with my other paper. And then re-check density if they do not...}
 	}
 	\label{tab: XrayAGprop}
 	\begin{tabular}{lccccc}
    \hline
       \hline
       \\[-2.5mm]
   \textbf{GRB} & \textbf{$t_o$} & \textbf{$\alpha_X$} & \textbf{$\beta_X$}  & \textbf{$F_{X,o}$} & \textbf{$n_\textrm{min}$} \\
   & \textbf{(s)} & & & \textbf{($10^{-11}$ erg cm$^{-2}$ s$^{-1}$)} & \textbf{(cm$^{-3}$)}\\
    \hline
 091109B & $160^{+120}_{-70}$ & $0.7\pm0.1$ & $0.9^{+0.5}_{-0.2}$ & $1.0\pm0.2$ & \\[0.9mm]
 101224A & $630^{+780}_{-540}$ & -- & -- & $0.02\pm0.01$ & $3.6\times 10^{-6}$ \\[0.9mm]
 110112A & $190\pm100$  & $1.06\pm0.10$ & $1.3^{+0.5}_{-0.4}$ & $1.4\pm0.4$ & $1.4\times 10^{-3}$ \\[0.9mm]
110402A$^a$  & $590\pm40$ & $0.4\pm0.2$ & $0.89\pm0.25$ & $1.0\pm0.2$ & $4.0\times10^{-4}$ \\[0.9mm]
120305A  & $350^{+250}_{-90}$  & $1.6\pm0.5$ & $1.9\pm0.7$ & $1.1\pm0.2$ & $2.0\times 10^{-5}$ \\[0.9mm]
 120630A & $175_{-80}^{+120}$ & $1.6\pm0.5$ & $0.7^{+0.6}_{-0.3}$ & $0.48\pm0.11$ & $9.0\times 10^{-5}$\\[0.9mm]
 130822A & -- & $\sim$\,$8.0$ & $1.1^{+1.8}_{-0.9}$ & -- & -- \\[0.9mm]
 130912A & $160\pm20$ & $1.2\pm0.08$ & $0.5\pm0.15$ & $24\pm5$ & $2.1\times 10^{-3}$ \\[0.9mm]
 131004A & $120^{+40}_{-50}$ & $0.96\pm0.07$ & $0.97\pm0.18$ & $3.8\pm0.8$ & $1.5\times10^{-3}$ \\[0.9mm]
140129B  & $330\pm10$  & $1.2\pm0.1$ & $1.0\pm0.2$ & $5.6\pm1.3$ & $1.0\times 10^{-3}$ \\[0.9mm]
 140516A & $200^{+2400}_{-110}$ & -- & $0.4^{+1.0}_{-0.4}$ & $0.06\pm0.02$ & $9.0\times 10^{-5}$ \\[0.9mm]
140622A  & $300^{+1100}_{-100}$ & $3.0\pm1.0$ & $0.6^{+0.7}_{-0.4}$ & $0.04\pm0.01$ & $1.8\times 10^{-5}$ \\[0.9mm]
 140930B & $187\pm4$  & $1.17\pm0.12$ & $0.7\pm0.2$ & $40\pm5$ & $1.4\times 10^{-3}$ \\[0.9mm]
 150423A & $110\pm30$ & $1.01\pm0.10$ & $0.51^{+0.36}_{-0.25}$ & $1.6\pm0.4$ & $2.6\times 10^{-4}$ \\[0.9mm]
 150831A & $240^{+90}_{-40}$ & $1.1\pm0.2$ & $0.8^{+0.5}_{-0.4}$ & $1.5\pm0.4$ & $2.4\times 10^{-5}$ \\[0.9mm]
 151229A & $76\pm4$ & $0.54\pm0.12$ & $1.03\pm0.14$ & $33\pm4$ & $1.2\times 10^{-1}$ \\[0.9mm]
 160408A & $300\pm20$ & $1.6\pm0.4$ & $1.0\pm0.4$ & $3.2\pm0.7$ & $1.8\times 10^{-4}$ \\[0.9mm]
 160410A$^a$ & $360\pm8$ & $1.2\pm0.2$ & $0.33\pm0.10$ & $8.0\pm2.0$ & $2.6\times10^{-3}$ \\[0.9mm]
 160525B & $73\pm3$  & $1.4\pm0.1$ & $0.95\pm0.25$ & $10.5\pm3.0$ & $6.6\times 10^{-3}$ \\[0.9mm]
 160601A & $270^{+420}_{-190}$ & $0.44\pm0.15$ & $1.0^{+0.8}_{-0.5}$ & $0.10\pm0.02$ & $8.2\times10^{-6}$ \\[0.9mm]
160927A  & $130^{+30}_{-50}$  & $1.02\pm0.09$  & $0.65^{+0.30}_{-0.15}$ &$1.9\pm0.4$ & $1.1\times10^{-4}$ \\[0.9mm]
 170127B & $130^{+50}_{-30}$ & $1.9\pm0.7$ & $0.6^{+0.4}_{-0.2}$ & $6.0\pm1.0$ & $7.3\times 10^{-4}$ \\[0.9mm]
  170428A & $800^{+150}_{-100}$ & $1.0\pm0.2$ & $2.0^{+1.3}_{-1.0}$ & $0.25\pm0.06$ & $1.6\times 10^{-5} $\\[0.9mm]
 170728A & $250^{+70}_{-50}$ & $0.90\pm0.10$ & $1.1^{+0.3}_{-0.1}$ & $1.0\pm0.2$ &  $1.2\times 10^{-4}$ \\[0.9mm]
 170728B$^a$ & $460\pm2$  & $0.6\pm0.1$ & $1.0\pm0.1$ & $37\pm7$ & $7.5\times 10^{-4}$ \\[0.9mm]
  171007A$^a$ &  $370^{+1500}_{-130}$ & $0.7^{+0.2}_{-0.7}$  & $0.36^{+0.49}_{-0.25}$ & $0.17\pm0.03$ & $8.0\times10^{-7}$ \\[0.9mm]
 180618A$^a$ & $69.1\pm0.6$  & $0.82\pm0.15$ & $0.88\pm0.08$ & $130\pm20$ & \textcolor{red}{XX} \\[0.9mm]
 180727A & $230^{+70}_{-50}$ & $1.0\pm0.4$ & $0.8\pm0.4$ & $1.5\pm0.3$ & $3.0\times 10^{-5}$ \\[0.9mm]
 180805B$^a$ & $1300^{+90}_{-130}$ & $1.04\pm0.16$ & $1.1\pm0.5$ & $0.25\pm0.07$ & $3.0\times 10^{-6}$ \\[0.9mm]
 191031D & $120\pm20$ & $2.0\pm0.2$  & $0.95^{+0.31}_{-0.16}$ & $2.9\pm0.7$ & \textcolor{orange}{XX} \\[0.9mm]
 200411A & $280^{+90}_{-80}$ & $0.9\pm0.2$ & $0.7\pm0.2$  & $1.0\pm0.2$ & $2.3\times10^{-4}$ \\[0.9mm]
     \hline
    \end{tabular}
\begin{flushleft}
    \quad \footnotesize{$^a$ Short GRB with extended emission.} \\
    \quad \footnotesize{$^b$ The early X-ray lightcurve of this GRB does not fit the criteria outlined by \citet{OConnor2020}.} \\
\end{flushleft}
\end{table*}


==> table_test.tex <==
\begin{table*}
 	\centering
 	\caption{Log of short GRB host galaxy observations. \brendan{Make another table for the spectroscopic observations?}
 	}
 	\label{tab: observations}
 	\begin{tabular}{lccccccccccc}
    \hline
       \hline 
       \\[-2.5mm]
   \textbf{GRB} & \textbf{$T_{90}^c$} & \textbf{RA} & \textbf{Dec} &\textbf{Obs. Date}  &   \textbf{Telescope} & \textbf{Instrument} & \textbf{Filter} & \textbf{Exp.} &  \textbf{AG Image}$^{b}$ & \textbf{AB Mag} &\textbf{$A_\lambda$}  \\
   & \textbf{(s)} &  \textbf{(J2000)} & \textbf{(J2000)} & \textbf{(UT)} & & & & \textbf{(s)} & &   & \textbf{(mag)} \\
    \hline
%    090621B &  0.14 &  20:53:53.17 &  69:01:41.4	 &  06-14-2014 3:27:41 & LDT & LMI  & \textit{r} & 3780  & ... & 1.37 \\
%    ... &  ... & ... & ... &  10-25-2014 06:10:33 & Keck & LRIS  & \textit{G} & 2700  & ...  & ... \\
%    ... &  ... & ... & ...  & 10-25-2014 06:16:45  & Keck  & LRIS & \textit{R} & 2000  & ...  & ...   \\
%    \hline
   091109B & 0.3 & 07:30:56.61 & -54:05:22.85 & 11-10-2009   & VLT & FORS2  & \textit{R}  & 3600 & Y &   0.45 \\
   ... & ... & ... & ... & 02-26-2012 & \textit{HST} & WFC3 & \textit{F160W} & 5600 & ... &   ...\\
   ... & ... & ... & ... & 11-01-2016  & \textit{HST} & WFC3 & \textit{F110W} & 5600 & ... &   ...\\
   \hline
   110112A & 0.5 & 21:59:43.85 & 26:27:23.9 &  01-12-2011  & WHT & ACAM &  \textit{i} & 900 & Y & 0.16\\
      ... & ... & ... & ... & 10-13-2016   & \textit{HST} & WFC3 & \textit{F110W} & 5200 & ... &   ...\\
   \hline
  110402A$^{a}$  & 60.9 & 21:59:43.85 & 26:27:23.9 & \textcolor{red}{xxx} & \textit{Swift} & UVOT & \textcolor{red}{xxx} & \textcolor{red}{xxx} &  Y & 0.05\\
   ... & ... & ... & ... & 08-03-2020  & Gemini & GMOS-N & \textit{r} & 900 & ... &  ...  \\
     ... & ... & ... & ... & 05-05-2021  & LDT & LMI & \textit{i} & 1500 & ... &  ...  \\
  ... & ... & ... & ... & 05-06-2021  & LDT & LMI & \textit{z} & \textcolor{red}{xxx} & ... &  ...  \\
    \hline
  120305A  & 0.1 & 03:10:08.68 & 28:29:31.0 & 03-06-2014	  & LDT  & LMI & \textit{r} & 2700 & ... & 1.15 \\
  ... & ... & ... & ... & 10-25-2014	&   Keck& LRIS&\textit{G}& 3000 & ... & ... \\
    ... & ... & ... & ... & 10-25-2014	&  Keck& LRIS&\textit{R} & 2750 & ... & ... \\
  \hline
  120630A  & 0.6 & 23:29:11.07 & 42:33:20.3 & 07-01-2012   & Gemini  & GMOS-N & \textit{r} & 500 & ... &  0.29 \\
    ... & ... & ... & ... &07-01-2012& Gemini & GMOS-N & \textit{i} & 500 & ... &  ... \\
      ... & ... & ... & ... &07-01-2012 & Gemini & GMOS-N & \textit{z} & 500 & ... &  ... \\
  ... & ... & ... & ... & 09-05-2014  & LDT & LMI & \textit{r} & 700 & ... &  ... \\
 ... & ... & ... & ... &09-05-2014 & LDT & LMI & \textit{i} & 400 & ... &  ... \\
  ... & ... & ... & ... &2014-09-05	 & LDT & LMI & \textit{z} & 800 & ... &  ... \\
  ... & ... & ... & ... &10-25-2014 & Keck & LRIS & \textit{R} & 3300 & ... &  ... \\
    ... & ... & ... & ... &10-25-2014 & Keck & LRIS & \textit{G} & 3600 & ... &  ... \\
 %  \hline
 %    \textcolor{magenta}{121226A} &  & & & & & & & & & \\
 %  ... & ... & ... & ... & &  &  &  & & ... & ... \\
  \hline
  130822A  & 0.04 & 01:51:41.27 & -03:12:31.7 & 08-23-2013	 & Gemini & GMOS-N & \textit{i} & 600 & ... &  0.08 \\
  ...  & ... & ... & ... & 10-25-2014 & Keck & LRIS & \textit{G} & 3000 & ... & ... \\
   ...  & ... & ... & ... & 10-25-2014	 & Keck & LRIS & \textit{R} & 2750 & ... & ... \\
  \hline
  130912A  & 0.28 & 03:10:22.23 & 13:59:48.7 & 09-13-2013  & WHT & ACAM & \textit{i} & 900 & Y & 0.76 \\
  ...  & ... & ... & ... & 02-25-2014  & LDT & LMI & \textit{r} & 2700 & ... & ... \\
  ...  & ... & ... & ... &10-25-2014   & Keck & LRIS &  \textit{G} & 2400 & ... & ... \\
 ...  & ... & ... & ... & 10-25-2014  & Keck & LRIS & \textit{R}  & 2750  & ... & ... \\
  ...  & ... & ... & ... & 01-09-2017  & \textit{HST} & WFC3 & \textit{F110W} & 5200 & ... & ... \\
   \hline
    131004A   & 1.54 & 19:44:27.08& -02:57:30.2 & \textcolor{red}{xxx} & \textit{Swift} & UVOT & \textit{wh} & \textcolor{red}{xxx} & Y & 0.76 \\
      ...& ... &...& ...& \textcolor{red}{xxx}  & Keck & MOSFIRE & \textit{$K_s$} & \textcolor{red}{xxx}  & ... &  \\
     ...  & ... & ... & ... & 10-11-2016 & \textit{HST} & WFC3 & \textit{F110W} & 5212 & ... & 0.77 \\
  \hline
  140930B  & 0.84 &  00:25:23.4 &24:17:41.7 &09-30-2014	& WHT & ACAM & \textit{r} & 3800 & Y & 0.08 \\ 
     ...  & ... & ... & ... & & LDT & &  & & ... & ... \\
   ...  & ... & ... & ... & 08-01-2020 & Gemini & GMOS-N &  \textit{r}& 1650 & ... & ... \\
  \hline
  150423A  & 0.08 & 14:46:18.86 & 12:17:00.70 &  04-23-2015 08:02:19 & VLT & FORS2 & \textit{R} & 300 & Y & 0.08 \\
    ...  & ... & ... & ... & 02-03-2017  & \textit{HST} & WFC3 & \textit{F110W} & 5200 & ... & ... \\
  \hline
  151229A  & 1.44 &21:57:28.78& 	-20:43:55.2 & 03-08-2019 & LDT & LMI & \textit{r}&1200 & ... & 0.07 \\
  ...& ... &...& ...& 07-30-2019   & Gemini &GMOS-S & \textit{z}&1920 & ... &  \\
  ...& ... &...& ...& 10-15-2019   & Keck & MOSFIRE & \textit{Y} & 1340 & ... &  \\
  ...& ... &...& ...& 08-11-2020   & Gemini & GMOS-N & \textit{r}&2250 & ... & ...  \\
  ...& ... &...& ...& 06-16-2021  & LDT & LMI & \textit{i}& 900 & ... & ...  \\
  \hline
  160601A  & 0.12 & 15:39:43.97 & 64:32:30.5 & 06-02-2016  &  Gemini & GMOS-N & \textit{r} & 900 & Y & 0.07 \\
   ... & ... & ... & ... & 06-03-2016  & LDT  & LMI & \textit{r} & 720 & ... & ...\\
 ... & ... & ... & ... & 08-01-2020	 & Gemini & GMOS-N & \textit{r} & 1800 & ... & ... \\
  \hline
  160927A  & 0.48 & 17:04:58.22 & 17:19:54.9 & 09-28-2016  & GTC & OSIRIS & \textit{r} & 1915 & Y & 0.21 \\
   ... & ... & ... & ... & 02-23-2017   & GTC   & OSIRIS  &\textit{r}  & 1200 & ... & ... \\
   ... & ... & ... & ... & 05-20-2018    & LDT  &  LMI & \textit{r} & 300 & ... & ... \\
   ... & ... & ... & ... & 08-01-2020    & Gemini & GMOS-N & \textit{i} & 720 & ... & ... \\
  % ... & ... & ... & ... & &  &  &  & & ... & ... \\
  \hline
   170127B & 0.5  &01:19:54.47 &-30:21:28.6 & 2018-01-27 & Gemini & GMOS-S & \textit{g} & 1800 &... & 0.06 \\
    ... & ... & ... & ... & 2018-10-06 & Keck & LRIS &\textit{G}  & 2520 & ... & ... \\
    ... & ... & ... & ... & 2018-10-06  & Keck & LRIS &\textit{R}  & 1720 & ... & ... \\
    ... & ... & ... & ... & 2019-09-04  & Keck & LRIS &\textit{G}  & 1920 & ... & ... \\
    ... & ... & ... & ... & 2019-09-04 & Keck & LRIS &\textit{I}  & 1600 & ... & ... \\
    ... & ... & ... & ... & 2019-10-15  & Keck & MOSFIRE &\textit{J}  & 2010 & ... & ... \\
    ... & ... & ... & ... & 01-30-2021 & Gemini & GMOS-S &\textit{z}  & 1440 & ... & ... \\
    \hline
   171007A$^a$ & 105 &09:02:24.14 & 42:49:08.8 & 01-09-2020  & LDT & LMI & \textit{r}  & 1200 & ... &  0.06\\
    ... & ... & ... & ... & 02-01-2021  & Gemini  & GMOS-N  & \textit{i}  & 1440 & ... & ... \\
      \hline
 170728A  & 1.3  &03:55:33.17 & 12:10:54.7 & \textcolor{red}{xxx} & \textit{Swift} & UVOT & & & Y & 0.65 \\
    ... & ... & ... & ... & 01-14-2018  & Keck & LRIS  & \textit{G}  & 1380 & ... & ... \\
    ... & ... & ... & ... & 01-14-2018 & Keck & LRIS  & \textit{R}  & 1380 & ... & ... \\
    ... & ... & ... & ... &  \textcolor{red}{xxx} & LDT & LMI  &   \textit{r} & & ... & ... \\
 %       \hline
 % \textcolor{magenta}{180618A$^a$} &  & & & & & & & & & \\
 %  ... & ... & ... & ... & &  &  &  & & ... & ... \\
         \hline
   191031D & 0.3 &18:53:09.57 &47:38:38.8 & 11-02-2019  & Gemini & GMOS-N & \textit{r} & 720 & ... & 0.2 \\
    ... & ... & ... & ... & 11-03-2019 & LDT  & LMI  & \textit{g}  &1200& ... & ... \\
    ... & ... & ... & ... & 11-03-2019 & Gemini  & GMOS-N &  \textit{i} & 355 & ... & ... \\
    ... & ... & ... & ... & \textcolor{red}{xxx} & LDT & LMI  &   \textit{g} & & ... & ... \\
    ... & ... & ... & ... &\textcolor{red}{xxx} & LDT & LMI  &   \textit{i} & & ... & ... \\
    ... & ... & ... & ... &\textcolor{red}{xxx} & LDT & LMI  &  \textit{z} & & ... & ... \\
    ... & ... & ... & ... &\textcolor{red}{xxx} & LDT & LMI  &  \textit{Y} & & ... & ... \\
\hline
  200411A  & 0.33  &03:10:39.39	 & -52:19:03.4 &01-25-21 & Gemini & GMOS-S & \textit{r} & 1800 & ... & 0.06\\
 % \hline
 %   & & & & & & & & & &  \\
 %   & & & & & & & & & &  \\
 %   & & & & & & & & & &  \\
 %   & & & & & & & & & & \\
 %   & & & & & & & & & & \\
 %   & & & & & & & & & & \\
     \hline
    \end{tabular}
\begin{flushleft}
    \quad \footnotesize{$^a$ Short GRB with extended emission.} \\
    \quad \footnotesize{$^b$ Afterglow image used for relative alignment.}\\
    \quad \footnotesize {$^c$ $T_{90}$ values were retrieved from the \textit{Swift} BAT GRB catalog \citep{Lien2016}.}\\
   % \quad \footnotesize {$^d$ Galactic extinction in the direction of the burst \citep{Schlafly2011}.}\\
\end{flushleft}
\end{table*}
